World to Code: Multi-modal Data Generation via Self-Instructed Compositional Captioning and Filtering

Recent advances in Vision-Language Models (VLMs) and the scarcity of high-quality multi-modal alignment data have inspired numerous researches on synthetic VLM data generation. The conventional norm in VLM data construction uses a mixture of specialists in caption and OCR, or stronger VLM APIs and expensive human annotation. In this paper, we present World to Code (W2C), a meticulously curated multi-modal data construction pipeline that organizes the final generation output into a Python code format. The pipeline leverages the VLM itself to extract cross-modal information via different prompts and filter the generated outputs again via a consistency filtering strategy. Experiments have demonstrated the high quality of W2C by improving various existing visual question answering and visual grounding benchmarks across different VLMs. Further analysis also demonstrates that the new code parsing ability of VLMs presents better cross-modal equivalence than the commonly used detail caption ability. Our code is available at https://github.com/foundation-multimodal-models/World2Code.

==> latex/tables/show_cases.tex <==

\begin{table}[tp]
\caption{OCR and captions generation comparison based on LLaVA-NEXT-13B model.}
\begin{minipage}{0.99\textwidth}

\scalebox{0.98}{
\begin{tabular}{l  }
\toprule
% \hline
\multicolumn{2}{l}{\bf \textit{OCR cases}}  \\
\hline
& \includegraphics[height=0.6cm]{Styles/figures/cases/ocr_case1.png} &\includegraphics[height=0.6cm]{Styles/figures/cases/ocr_case2.png} \\
\textbf{\textit{Question:}} & What is written in the image? & What is the number in the image?\\
Baseline: &The word "\red{consciousness}" is written in the image. &The word "\red{world}" is written in the image.\\
\ours: &The word "\green{construction}" is written in the image. &The word "\green{would}" is written in the image.\\
\midrule
% \hline
& \includegraphics[height=2.5cm]{Styles/figures/cases/ocr_case3.png} &\includegraphics[height=2.5cm]{Styles/figures/cases/ocr_case4.png} \\
\textbf{\textit{Question:}} & What is the Mosman Manly exit going to? & How many items purchased from Amazon?\\

Baseline: &The mosman manly exit is going to \red{mosman}. &There are \red{2.43 million} items purchased from amazon.\\
\ours: &The mosman manly exit is going to \green{chatswood epping}. &\green{902k}.\\
\midrule
% \hline
\multicolumn{2}{l}{\bf \textit{Short caption cases}}  \\
% \hline
\midrule
& \includegraphics[height=2.5cm]{Styles/figures/cases/short_cap_case1.png} &\includegraphics[height=2.5cm]{Styles/figures/cases/short_cap_case2.png} \\
\textbf{\textit{Question:}} & Provide a one-sentence caption for the provided image. & Provide a one-sentence caption for the provided image.\\
Baseline: &A red background with a sun and birds and the words Sibelius Symphonies No 2 \& 5. &A book is open to a page with a picture of \red{a man on a horse}.\\
\ours: &A \green{cd cover} for Sibelius Symphonies Nos 2 \& 5. &A book is open to a page with a picture of \green{two men on horses}.\\
\midrule
% \hline
& \includegraphics[height=2.5cm]{Styles/figures/cases/short_cap_case6.jpg} &\includegraphics[height=2.5cm]
{Styles/figures/cases/short_cap_case7.jpg} \\
\textbf{\textit{Question:}} & Provide a one-sentence caption for the provided image. & Provide a one-sentence caption for the provided image.\\
Baseline: &A silver car is parked in front of a fence and a bus. &A person riding a horse with a cart attached to it.\\
\ours: &A silver car is parked behind a fence in front of a \green{trolley}. &A horse pulling a cart \green{with the number 8} on it.\\
\bottomrule
% \hline
\end{tabular}
}
\vspace{1mm}
% \vspace{-5mm}
\label{tab:ocr_cases}  
\end{minipage}
\end{table}
